Recall or Relearn? A Mixture of In-Context Experts for Recurring Concept Drift

Tabular foundation models (TFMs) are being applied to Web data streams such as network intrusion detection, where they adapt by updating the labelled rows of their context without retraining. When a past concept returns after leaving the context, a TFM faces a recall-or-relearn decision between restoring stored rows of the concept and relearning it from new labels. We propose MICE (Mixture of In-Context Experts), a training-free learner that cuts the stream into segments at detected changes. It merges a closed segment into a stored context when the TFM's estimated additional error on the segment is within a tolerance, under a capacity limit on stored contexts. A fast level weights the stored contexts and first-in-first-out (FIFO) windows by the log-loss of their predictions on the last labelled batch. We show that, with pure stored contexts and a margin condition, this fast level gains over relearning, in expected accuracy, the normalised positive area between the stored context's accuracy and the TFM's learning curve, up to a first-batch term. A slow level mixes the fast level's prediction with that of the FIFO window of the last labelled rows and bounds the discounted half-Brier regret of MICE against this window at every time. Learning curves measured beforehand predict the ordering of the observed recall gains. MICE outperforms reset, which empties the context at detected drifts, on grid streams with random boundary phases. Merging keeps fewer experts than pools that store every segment, and with fixed segmentation a time-matched snapshot pool matches MICE on the shifted grid. On real streams, MICE has the highest mean accuracy of all policies we compare.

==> tab_main_rows_r10.tex <==
\multicolumn{14}{l}{\emph{Trained stream learners}} \\
ARF~\citep{gomes2017arf} & 73.4 & 58.4 & 85.4 & 6.0 & 18.7 & $-$37.5 & 67.7 & 65.6 & 83.8 & 11.2 & 22.9 & 88.0 & 98.39 \\
SRP~\citep{gomes2019srp} & 76.6 & 62.3 & 87.5 & 6.0 & 16.7 & $-$19.8 & 69.5 & 68.1 & 84.7 & 8.8 & 21.6 & 86.4 & 98.57 \\
HAT~\citep{bifet2009hat} & 64.3 & 51.1 & 79.1 & 16.5 & 27.4 & $-$49.6 & 51.4 & 49.4 & 74.5 & 13.3 & 32.1 & 79.2 & 97.93 \\
Leveraging Bagging~\citep{bifet2010levbag} & 72.4 & 57.3 & 85.9 & 5.1 & 19.1 & $-$34.6 & 62.0 & 60.6 & 82.4 & 7.2 & 24.9 & 85.9 & 98.39 \\
ADWIN Bagging~\citep{bifet2009new} & 65.1 & 51.5 & 81.4 & 7.8 & 24.0 & $-$50.1 & 51.2 & 49.2 & 76.1 & 9.4 & 30.8 & 77.0 & 97.91 \\
Learn++.NSE~\citep{elwell2011nse} & 67.7 & 51.2 & 82.8 & 8.5 & 22.3 & $-$41.0 & 61.6 & 60.0 & 81.2 & 30.0 & 33.6 & 84.1 & 94.86 \\
FSNet~\citep{pham2023fsnet} & 77.3 & 64.9 & 88.1 & 4.6 & 15.6 & $-$26.7 & 62.7 & 61.3 & 80.4 & 8.4 & 24.8 & 87.5 & 98.21 \\
OneNet~\citep{zhang2023onenet} & 77.8 & 65.1 & 88.1 & 4.2 & 15.2 & $-$22.1 & 62.4 & 60.9 & 80.1 & \second{7.0} & 24.6 & 87.6 & 97.19 \\
ShifTS~\citep{zhao2026shifts} & 73.4 & 59.9 & 84.6 & 3.5 & 17.7 & $-$30.4 & 51.1 & 47.0 & 71.7 & \first{6.0} & 29.3 & 76.4 & 97.72 \\
ADAPT-Z~\citep{huang2026adaptz} & 65.6 & 50.7 & 80.1 & 5.6 & 22.3 & $-$52.3 & 50.1 & 46.2 & 70.7 & \first{6.0} & 30.0 & 78.1 & 97.43 \\
\midrule
\multicolumn{14}{l}{\emph{In-context policies, frozen TabPFN}} \\
FIFO & \second{83.3} & 73.5 & 89.9 & 1.7 & \third{11.6} & -- & 61.9 & 60.9 & 83.7 & 16.7 & 25.1 & 87.6 & 98.57 \\
LTM~\citep{lourenco2026streams} & 82.6 & 72.1 & \first{91.0} & 1.5 & 11.9 & $-$2.7 & 62.2 & 61.4 & 84.8 & 16.0 & 24.5 & 87.6 & 98.21 \\
Reset~\citep{gama2004ddm} & 81.5 & 71.3 & 88.5 & 2.6 & 12.9 & $-$9.6 & 84.1 & 83.8 & 91.4 & 7.3 & 13.1 & 94.8 & 98.49 \\
Window ensemble & \third{83.0} & 73.0 & 89.5 & \second{1.2} & 11.7 & $-$1.4 & 81.6 & 81.0 & 90.8 & 8.7 & 14.9 & 94.6 & 98.44 \\
Drift-Resilient TabPFN~\citep{helli2024drift} & 81.7 & 68.7 & 88.4 & 3.0 & 12.9 & $-$4.2 & 76.4 & 75.6 & 87.4 & 9.8 & 17.9 & 93.7 & 98.37 \\
\midrule
\multicolumn{14}{l}{\emph{Ours}} \\
\textbf{\method{} (full, detected seg.)} & \first{83.8} & \first{74.4} & \second{90.7} & \third{1.3} & \first{11.2} & \second{$-$0.23} & \third{86.4} & \third{86.0} & \second{92.4} & 9.9 & \third{12.6} & \third{95.0} & \third{98.59} \\
\method{}, fixed segments & \first{83.8} & \second{74.3} & \third{90.5} & \third{1.3} & \first{11.2} & \third{$-$0.25} & \third{86.4} & \third{86.0} & \third{92.3} & 10.1 & 12.7 & \third{95.0} & \second{98.60} \\
\method{}, fixed segments, $\eta_2=10$ & \first{83.8} & \third{74.2} & \third{90.5} & \first{1.1} & \first{11.2} & \first{$-$0.08} & \second{86.6} & \second{86.3} & \first{93.6} & \second{7.0} & \second{11.5} & \second{95.2} & \first{98.61} \\
\method{} w/o slow level (fixed seg.) & \second{83.3} & 73.4 & 90.3 & 1.5 & \second{11.5} & $-$2.3 & \first{86.8} & \first{86.5} & \first{93.6} & \third{7.1} & \first{11.4} & \first{95.3} & 98.50 \\

